CommonScenes: Generating Commonsense 3D Indoor Scenes with Scene Graph Diffusion

Controllable scene synthesis aims to create interactive environments for various industrial use cases. Scene graphs provide a highly suitable interface to facilitate these applications by abstracting the scene context in a compact manner. Existing methods, reliant on retrieval from extensive databases or pre-trained shape embeddings, often overlook scene-object and object-object relationships, leading to inconsistent results due to their limited generation capacity. To address this issue, we present CommonScenes, a fully generative model that converts scene graphs into corresponding controllable 3D scenes, which are semantically realistic and conform to commonsense. Our pipeline consists of two branches, one predicting the overall scene layout via a variational auto-encoder and the other generating compatible shapes via latent diffusion, capturing global scene-object and local inter-object relationships in the scene graph while preserving shape diversity. The generated scenes can be manipulated by editing the input scene graph and sampling the noise in the diffusion model. Due to lacking a scene graph dataset offering high-quality object-level meshes with relations, we also construct SG-FRONT, enriching the off-the-shelf indoor dataset 3D-FRONT with additional scene graph labels. Extensive experiments are conducted on SG-FRONT where CommonScenes shows clear advantages over other methods regarding generation consistency, quality, and diversity. Codes and the dataset will be released upon acceptance.

==> sections/dataset.tex <==
\section{SG-FRONT Dataset}

\input{tex/figure/qual_comp}
Due to the lack of high-quality scene graph datasets providing object meshes, we construct \emph{SG-FRONT} based on a 3D synthetic dataset 3D-FRONT~\cite{3dfront} that offers professionally designed layouts and objects.
Our main contribution is to add well-annotated scene graph labels to 3D-FRONT.
The annotation labels can be grouped into three categories \textbf{\textit{spatial/proximity, support, and style}}. 
The spatial relationships are based on a set of relationship checks between the objects, which control the object bounding box location (\texttt{left/right}, \texttt{front/behind}), the comparative volumes (\texttt{bigger/smaller}), and heights (\texttt{lower/higher}). 
The support relationships include directed structural support, such as \texttt{close by}, \texttt{above}, and \texttt{standing on}.
Thresholds for these labels are iterated and set by the annotators.
Finally, style relationships include the object attributes to assign labels such as \texttt{same material as}, \texttt{same shape as}, or \texttt{same super-category as}.
SG-FRONT contains around 45K samples from three different indoor scene types, covering 15 relationship types densely annotating scenes.
More details are provided in the Supplementary Material.


==> tex/table/others.tex <==




\iffalse
\begin{table*}[h!]
    \centering
    \scalebox{0.75}{
    \begin{tabular}{lc|c|cccc|cccc}
        \midrule \midrule
         \multirow{2}{*}{Method} &  \multirow{2}{*}{Shape Model} & Shape & \multicolumn{4}{c|}{Generation} & \multicolumn{4}{c}{Manipulation} \\
        & & Representation & Size & Location & Angle & Shape & Size & Location & Angle & Shape \\
        \midrule  \midrule
        3D-SLN~\cite{Luo_2020_CVPR} & Retrieval & \multirow{2}{*}{3RScan Data} & 0.026 & 0.064 & 11.833	& \textbf{0.088} & 0.001 & 0.002 & 0.290 & 0.002 \\
        Progressive & -- & & 0.009 & 0.011  & 1.494 & -- & 0.008 & 0.008 &  1.559 & --  \\
        \midrule
        Graph-to-Box & Graph-to-Shape & \multirow{2}{*}{AtlasNet~\cite{groueix2018atlas}} & 0.009 & 0.024 & 1.869 & 0.000 &  0.007 &0.019 &  2.920 & 0.000  \\
        \multicolumn{2}{c|}{Graph-to-3D}  & & \textbf{0.097} & \textbf{0.497}  & \textbf{20.532} &  0.005 & \textbf{0.037} & \textbf{0.061} & \textbf{14.177} & 0.007\\
        \midrule
        Graph-to-Box & Graph-to-Shape & \multirow{2}{*}{DeepSDF~\cite{park2019deepsdf}} & 0.009 & 0.024 & 1.895 & 0.011 & 0.005 & 0.019 & 3.391 & 0.014 \\
        \multicolumn{2}{c|}{Graph-to-3D} & & 0.091 & 0.485 & 19.203 & 0.015 & 0.015 & 0.035 & 9.364 & \textbf{0.016} \\
        \midrule
        Ours & Retrieval & DeepSDF & \\
        Ours & Retrieval & SDFusion & \\
        \multicolumn{2}{c|}{Ours full} & SDFusion & \\
        \midrule \midrule
    \end{tabular}}
    \caption{Comparison on diversity results (std) on the generation (left) and manipulation tasks (right), computed as standard deviation over location and size in meters and angles in degrees. For shape we report the average chamfer distance between consecutive generations.}
    \label{tab:diversity_3dssg}
\end{table*}
\fi


\iffalse
\begin{table*}[h!]
    \centering
    \scalebox{0.75}{
        \begin{tabular}{ll|c|ccc|ccc|ccc}
            \midrule \midrule
            \multirow{2}{*}{Layout Model} & \multirow{2}{*}{Shape Model} & Shape & \multicolumn{3}{c|}{Recall Objects} &\multicolumn{3}{c|}{Recall Predicate} & \multicolumn{3}{c}{Recall Triplets} \\ 
            & & Representation & Top 1 & Top 5 & Top 10 & Top 1 & Top 3 & Top 5 & Top 1 & Top 50 & Top 100 \\
            \midrule \midrule
            3D-SLN \cite{Luo_2020_CVPR} & Retrieval & - &  \\
            %Progressive & Retrieval & &  \\
            \midrule
            Graph-to-Box & Graph-to-Shape &\multirow{2}{*}{DeepSDF~\cite{park2019deepsdf}} &  \\
            \multicolumn{2}{c|}{Graph-to-3D}  &  &  \\
            \midrule
             \multicolumn{3}{c|}{3D-FRONT data}  & 
             \\
            \midrule
            \midrule

        \end{tabular}
    }
    \caption{Scene graph prediction accuracy on \textbf{3D-FRONT}, using the SGPN model from \cite{3DSSG2020}, measured as top-k recall for object, predicate and triplet prediction (higher is better). }
    \label{tab:sgpn_3dfront}
\end{table*}
\fi



\iffalse
\begin{table*}[h!]
    \centering
    \scalebox{0.75}{
    \begin{tabular}{l|c|cccc|cccc}
        \midrule \midrule
         \multirow{2}{*}{Method} & Shape & \multicolumn{4}{c|}{Generation} & \multicolumn{4}{c}{Manipulation} \\
        & Representation & Size & Location & Angle & Shape & Size & Location & Angle & Shape \\
        \midrule  \midrule
        3D-SLN~\cite{Luo_2020_CVPR} & 3D-Front Data & \\
        Graph-to-Box & SDFusion & \\
        Graph-to-3D & DeepSDF~\cite{park2019deepsdf} &  0.02 & 0.03 & 4.19 & 0.12 & 0.53 & 0.77 & 25.42 & 0.52\\
        \midrule
        Ours w/o DB & - & \\
        Ours & txt2shape & \\
        Ours & rel2shape & \\
        \midrule \midrule
    \end{tabular}}
    \caption{\textbf{3D-FRONT} Comparison on diversity results (std) on the generation (left) and manipulation tasks (right), computed as standard deviation over location and size in meters and angles in degrees. For shape we report the average chamfer distance between consecutive generations.($\times 0.01$)}
    \label{tab:diversity_3dfront}
\end{table*}
\fi


\iffalse
\begin{table}[h!]
    \centering
    \begin{tabular}{c|cccc }
    \toprule
         & E2 & CLIP & No end-to-end training & Metrics \\
     \midrule
         \textcircle{1} &  &  &  & 0.0 \\
         \textcircle{2} & \checkmark & & & 0.0 \\
         \textcircle{2} & \checkmark & \checkmark & & 0.0 \\
         \textcircle{2} &   & \checkmark & & 0.0 \\
         \textcircle{3} & \checkmark & \checkmark & \checkmark & 0.0 \\
     \bottomrule
    \end{tabular}
    \caption{Ablation studies}
    \label{tab:abl}
\end{table}
\fi

\begin{table*}[h!]
    \centering
    \scalebox{0.75}{
        \begin{tabular}{ll|c|ccc|ccc|ccc}
            \midrule \midrule
            \multirow{2}{*}{Layout Model} & \multirow{2}{*}{Shape Model} & Shape & \multicolumn{3}{c|}{Recall Objects} &\multicolumn{3}{c|}{Recall Predicate} & \multicolumn{3}{c}{Recall Triplets} \\ 
            & & Representation & Top 1 & Top 5 & Top 10 & Top 1 & Top 3 & Top 5 & Top 1 & Top 50 & Top 100 \\
            \midrule \midrule
            3D-SLN \cite{Luo_2020_CVPR} & Retrieval & \multirow{2}{*}{3RScan Data} & \textbf{0.56} & 0.81 & 0.88 & 0.50 & \textbf{0.82} & 0.86 & 0.15 & 0.57 & 0.82 \\
            Progressive & Retrieval & & 0.35 & 0.66 & 0.79 &  0.41 &  0.70 & 0.82 & 0.09 &  0.40 & 0.70 \\
            \midrule
            Graph-to-Box & Graph-to-Shape &  & 0.51 & 0.81 & 0.86 & 0.57 & 0.80 & 0.88 & \textbf{0.23} & 0.63 & 0.84 \\
            \multicolumn{2}{c|}{Graph-to-3D} &  & 0.54 & \textbf{0.84} & \textbf{0.90}  & \textbf{0.60} & \textbf{0.82} & \textbf{0.90} & 0.21 & \textbf{0.65} & \textbf{0.85} \\
            \midrule
            Graph-to-Box & Graph-to-Shape &\multirow{2}{*}{DeepSDF~\cite{park2019deepsdf}} & 0.47 & 0.74 & 0.83 & 0.57 & 0.80 & 0.87 & 0.14 & 0.57 & 0.81 \\
            \multicolumn{2}{c|}{Graph-to-3D}  &  & 0.51 & 0.80 & 0.88  & 0.58 & 0.80 & 0.89 & 0.19 & 0.59 & 0.83 \\
            \midrule
            Ours v2 & Retrieval & DeepSDF & \\
            Ours v2 & Retrieval & Text-to-SDFusion & \\
            \midrule
             \multicolumn{3}{c|}{3RScan data}  & 0.53 & 0.82 & 0.90 & 0.75 & 0.93 & 0.98 & 0.18 & 0.61 & 0.83
             \\
            \midrule
            \midrule

        \end{tabular}
    }
    \caption{Scene graph prediction accuracy on \textbf{3DSSG}, using the SGPN model from \cite{3DSSG2020}, measured as top-k recall for object, predicate and triplet prediction (higher is better). $^{\ddag}$Model trained with non-canonical objects, exhibiting significantly worse results.}
    \label{tab:sgpn_3dssg}
\end{table*}


